What Makes a Good Diffusion Planner for Decision Making?

Diffusion models have recently shown significant potential in solving decision-making problems, particularly in generating behavior plans -- also known as diffusion planning. While numerous studies have demonstrated the impressive performance of diffusion planning, the mechanisms behind the key components of a good diffusion planner remain unclear and the design choices are highly inconsistent in existing studies. In this work, we address this issue through systematic empirical experiments on diffusion planning in an offline reinforcement learning (RL) setting, providing practical insights into the essential components of diffusion planning. We trained and evaluated over 6,000 diffusion models, identifying the critical components such as guided sampling, network architecture, action generation and planning strategy. We revealed that some design choices opposite to the common practice in previous work in diffusion planning actually lead to better performance, e.g., unconditional sampling with selection can be better than guided sampling and Transformer outperforms U-Net as denoising network. Based on these insights, we suggest a simple yet strong diffusion planning baseline that achieves state-of-the-art results on standard offline RL benchmarks.

==> table.tex <==

\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cc|c|ccc|ccccc|ccccc|}
\hline
\multicolumn{1}{|c|}{\textbf{}}                                & \textbf{}                            & \cellcolor[HTML]{FFF2CC} IL & \multicolumn{3}{c|}{\cellcolor[HTML]{DDEBF7} Non-diffusion }                                                                                                   & \multicolumn{5}{c|}{\cellcolor[HTML]{E2EFDA}Diffusion Policies}                                                                                                                                                                                                                                                                             & \multicolumn{5}{c|}{\cellcolor[HTML]{FCE4D6}Diffusion   Planners}                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{Dataset}} & \cellcolor[HTML]{FFFFFF}\textbf{Env} & \cellcolor[HTML]{FFF2CC}BC        & \multicolumn{1}{c|}{\cellcolor[HTML]{DDEBF7}BCQ}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DDEBF7}CQL}                         & \cellcolor[HTML]{DDEBF7}IQL & \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}SfBC}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}DQL}                                & \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}DQL*}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}IDQL}                        & \cellcolor[HTML]{E2EFDA}IDQL* & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE4D6}Diffuser}                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE4D6}AdpDfsr}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE4D6}DD}         & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE4D6}HD}                                & \cellcolor[HTML]{FCE4D6} DV (ours) \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}Mixed}            & Kitchen                              & 47.5                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}8.1}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}51.0}                        & 51.0                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}45.4 ± 1.6}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}62.6 ± 5.1}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}55.1 ± 1.58}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}66.5}                        & 66.5 ± 4.1                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}52.5 ± 2.5}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}51.8 ± 0.8}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}75.0 ± 0.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}71.7 ±2.7}                         & 73.6 ± 0.1                          \\ \hline
\rowcolor[HTML]{F2F2F2} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{F2F2F2}Partial}          & Kitchen                              & 33.8                              & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}18.9}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}49.8}                        & 46.3                        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}47.9 ± 4.1}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}60.5 ± 6.9}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}65.5 ± 1.38}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}66.7}                        & 66.7 ± 2.5                    & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}55.7 ± 1.3}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}55.5 ± 0.4}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}56.5 ± 5.8} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}73.3 ± 1.4}                        & 94.0 ± 0.3                          \\ \hline
\rowcolor[HTML]{BDD7EE} 
\multicolumn{2}{|c|}{\cellcolor[HTML]{BDD7EE}\textbf{Average}}                                        & {\color[HTML]{000000} 40.7}       & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{000000} 13.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{000000} 50.4}} & {\color[HTML]{000000} 48.7} & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{000000} 46.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{000000} 61.6}}        & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{000000} 60.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{000000} 66.6}} & {\color[HTML]{000000} 66.6}   & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{000000} 54.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}53.7}        & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}65.8}       & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{000000} 72.5}}       & \textbf{83.8}                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}Large-diverse}    & Antmaze                              & {\color[HTML]{808080} 0.0}        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{808080} 2.2}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{808080} 61.2}} & {\color[HTML]{808080} 47.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}45.5 ± 6.6}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{808080} 56.6 ± 7.6}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}70.6 ± 3.7}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{808080} 67.9}} & 40.0 ± 11.4                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}27.3 ± 2.4}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}8.7 ± 2.5}   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.0 ± 0.0}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{808080} 83.6 ± 5.8}} & 80.0 ± 1.8                          \\ \hline
\rowcolor[HTML]{F2F2F2} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{F2F2F2}Large-play}       & Antmaze                              & {\color[HTML]{808080} 0.0}        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{808080} 6.7}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{808080} 53.7}} & {\color[HTML]{808080} 39.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}59.3 ± 14.3}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{808080} 46.4 ± 8.3}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}81.3 ± 3.1}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{808080} 63.5}} & 48.7 ± 4.7                    & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}17.3 ± 1.9}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}5.3 ± 3.4}   & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}0.0 ± 0.0}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{808080} --}}         & 76.4 ± 2.0                          \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}Medium-diverse}   & Antmaze                              & {\color[HTML]{808080} 0.0}        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{808080} 0.0}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{808080} 15.8}} & {\color[HTML]{808080} 70.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}82.0 ± 3.1}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{808080} 78.6 ± 10.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}82.6 ± 3.0}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{808080} 84.8}} & 83.3 ± 5.0                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2.0 ± 1.6}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}6.0 ± 3.3}   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}4.0 ± 2.8}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{808080} 88.7 ± 8.1}} & 87.4 ± 1.6                          \\ \hline
\rowcolor[HTML]{F2F2F2} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{F2F2F2}Medium-play}      & Antmaze                              & {\color[HTML]{808080} 0.0}        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{808080} 0.0}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{808080} 14.9}} & {\color[HTML]{808080} 71.2} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}81.3 ± 2.6}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{808080} 76.6 ± 10.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}87.3 ± 2.7}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{808080} 84.5}} & 67.3 ± 5.7                    & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}6.7 ± 5.7}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}12.0 ± 7.5}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}8.0 ± 4.3}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}--}                                & 89.0 ± 1.6                          \\ \hline
\rowcolor[HTML]{BDD7EE} 
\multicolumn{2}{|c|}{\cellcolor[HTML]{BDD7EE}\textbf{Average}}                                        & {\color[HTML]{808080} 0.0}        & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{808080} 2.2}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{808080} 36.4}} & {\color[HTML]{808080} 57.1} & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}67.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{808080} 64.6}}        & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}80.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}{\color[HTML]{808080} 75.2}} & 59.8                          & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}13.3}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}8.0}         & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}3.0}        & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}--}                                & \textbf{83.2}                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}Large}            & \cellcolor[HTML]{FFFFFF}Maze2D       & 5                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}6.2}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}12.5}                        & 58.6                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}74.4 ± 1.7}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}186.8 ± 1.7}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}90.1}                        & --                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}123}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}167.9 ± 5.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}128.4 ± 3.6}                       & 203.6 ± 1.4                         \\ \hline
\rowcolor[HTML]{F2F2F2} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{F2F2F2}Medium}           & Maze2D                               & 30.3                              & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}8.3}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}5.0}                         & 34.9                        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}73.8 ± 2.9}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}--}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}152.0 ± 0.8}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}89.5}                        & --                            & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}121.5}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}129.9 ± 4.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}--}         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}135.6 ± 3.0}                       & 150.7 ± 1.0                         \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}Umaze}            & \cellcolor[HTML]{FFFFFF}Maze2D       & 3.8                               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}12.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}5.7}                         & 47.4                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}73.9 ± 6.6}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}140.6 ± 1.0}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}57.9}                        & --                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}113.9}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}135.1 ± 5.8} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}155.8 ± 2.5}                       & 136.6 ± 1.3                         \\ \hline
\rowcolor[HTML]{BDD7EE} 
\multicolumn{2}{|c|}{\cellcolor[HTML]{BDD7EE}\textbf{Average}}                                        & 13.0                              & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}9.1}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}7.7}                         & 47.0                        & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}74.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}}                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}159.8}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}79.2}                        &                               & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}119.5}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}144.3}       & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}}           & \multicolumn{1}{c|}{\cellcolor[HTML]{BDD7EE}139.9}                             & \textbf{163.6}                      \\ \hline
\end{tabular}
} %
\caption{\textbf{Normalized performance of various offline-RL methods.} DQL* and IQL* are replicated results. Note that the latest version of Antmaze is v2, the previous results on AntMaze-v0 are denoted by gray fonts to differentiate. Data are Mean $\pm$ Standard Error (if available) over 500 episode seeds. The best average performance on each task set are marked in bold fonts. BC: vanilla imitation learning, BCQ: \cite{fujimoto2019off}, CQL: \cite{kumar2020conservative}, IQL: \cite{kostrikov2021offline}, SfBC: \cite{chen2023offline}, DQL: \cite{wang2023diffusion}, IDQL: \cite{hansen2023idql}, DQL* and IDQL*: replicated by \cite{dong2024cleandiffuser}, Diffuser: \cite{janner2022planning}, AdptDfsr: \cite{liang2023adaptdiffuser}, DD: \cite{ajay2022conditional}, HD: \cite{chen2024simple}.}
\label{table:score}
\end{table}


==> table_transpose.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{F2F2F2}}c 
>{\columncolor[HTML]{BDD7EE}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{F2F2F2}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{F2F2F2}}c 
>{\columncolor[HTML]{BDD7EE}}c |cccc|}
\hline
                                                                                                        & \textbf{Env}                     & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}Kitchen}                                                                               & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Antmaze}                                                                                                                                                                                                                                                                                                      & \multicolumn{4}{c|}{Maze2D}                                                                                                                                                                                         \\ \hline
Category                                                                                                & \textbf{Dataset}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}Mixed}     & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}Partial}   & \textbf{avg.} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}Large-div.}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}Large-play}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}Med.-div.}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}Med.-play}                      & \textbf{avg.}            & \multicolumn{1}{c|}{Large}                             & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}Med.}    & \multicolumn{1}{c|}{Umaze}                             & \cellcolor[HTML]{BDD7EE}\textbf{avg.} \\ \hline
\cellcolor[HTML]{DDEBF7}                                                                                & \cellcolor[HTML]{DDEBF7}BC       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}47.5}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}33.8}      & 40.7             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 0.0}}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 0.0}}      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 0.0}}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 0.0}}       & {\color[HTML]{A6A6A6} 0.0}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}5}         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}30.3}      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}3.8}       & \cellcolor[HTML]{BDD7EE}13.0             \\ \cline{2-14} 
\cellcolor[HTML]{DDEBF7}                                                                                & \cellcolor[HTML]{DDEBF7}BCQ      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}8.1}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}18.9}      & 13.5             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 2.2}}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 6.7}}      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 0.0}}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 0.0}}       & {\color[HTML]{A6A6A6} 2.2}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}6.2}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}8.3}       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}12.8}      & \cellcolor[HTML]{BDD7EE}9.1              \\ \cline{2-14} 
\cellcolor[HTML]{DDEBF7}                                                                                & \cellcolor[HTML]{DDEBF7}CQL      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}51.0}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}49.8}      & 50.4             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 61.2}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 53.7}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 15.8}}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 14.9}}      & {\color[HTML]{A6A6A6} 36.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}12.5}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}5.0}       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}5.7}       & \cellcolor[HTML]{BDD7EE}7.7              \\ \cline{2-14} 
\multirow{-4}{*}{\cellcolor[HTML]{DDEBF7}\begin{tabular}[c]{@{}c@{}}non-\\ diffusion\end{tabular}}      & \cellcolor[HTML]{DDEBF7}IQL      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}51.0}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}46.3}      & 48.7             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 47.5}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 39.6}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 70.0}}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 71.2}}      & {\color[HTML]{A6A6A6} 57.1} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}58.6}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}34.9}      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}47.4}      & \cellcolor[HTML]{BDD7EE}47.0             \\ \hline
\cellcolor[HTML]{E2EFDA}                                                                                & \cellcolor[HTML]{E2EFDA}SfBC     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}45.4$\pm$1.6}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}47.9$\pm$4.1}  & 46.7             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}45.5$\pm$6.6}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}59.3$\pm$14.3}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}82.0$\pm$3.1}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}81.3$\pm$2.6}                         & 67.0                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}74.4$\pm$1.7}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}73.8$\pm$2.9}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}73.9$\pm$6.6}  & \cellcolor[HTML]{BDD7EE}74.0             \\ \cline{2-14} 
\cellcolor[HTML]{E2EFDA}                                                                                & \cellcolor[HTML]{E2EFDA}DQL      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}62.6$\pm$5.1}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}60.5$\pm$6.9}  & 61.6             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 56.6$\pm$7.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 46.4$\pm$8.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 78.6$\pm$10.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 76.6$\pm$10.8}} & {\color[HTML]{A6A6A6} 64.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}--}        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}        & \cellcolor[HTML]{BDD7EE}                 \\ \cline{2-14} 
\cellcolor[HTML]{E2EFDA}                                                                                & \cellcolor[HTML]{E2EFDA}DQL*     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}55.1$\pm$1.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}65.5$\pm$1.4} & 60.3             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}70.6$\pm$3.7}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}81.3$\pm$3.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}82.6$\pm$3.0}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}87.3$\pm$2.7}                         & 80.5                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}186.8$\pm$1.7} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}152.0$\pm$0.8} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}140.6$\pm$1.0} & \cellcolor[HTML]{BDD7EE}159.8            \\ \cline{2-14} 
\cellcolor[HTML]{E2EFDA}                                                                                & \cellcolor[HTML]{E2EFDA}IDQL     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}66.5}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}66.7}      & 66.6             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 67.9}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 63.5}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 84.8}}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}{\color[HTML]{A6A6A6} 84.5}}      & {\color[HTML]{A6A6A6} 75.2} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}90.1}      & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}89.5}      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}57.9}      & \cellcolor[HTML]{BDD7EE}79.2             \\ \cline{2-14} 
\cellcolor[HTML]{E2EFDA}                                                                                & \cellcolor[HTML]{E2EFDA}IDQL*    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}66.5$\pm$4.1}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}66.7$\pm$2.5}  & 66.6             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}40.0$\pm$11.4}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}48.7$\pm$4.7}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}83.3$\pm$5.0}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}67.3$\pm$5.7}                         & 59.8                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}--}        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}        & \cellcolor[HTML]{BDD7EE}                 \\ \cline{2-14} 
\multirow{-6}{*}{\cellcolor[HTML]{E2EFDA}\begin{tabular}[c]{@{}c@{}}Diffusion\\ Policies\end{tabular}}  & \cellcolor[HTML]{E2EFDA}CEP      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}--}        & --               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}64.8$\pm$5.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}66.6$\pm$9.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}83.8$\pm$3.5}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}83.6$\pm$4.4}                         & 74.7                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}--}        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}        & \cellcolor[HTML]{BDD7EE}                 \\ \hline
\cellcolor[HTML]{FCE4D6}                                                                                & \cellcolor[HTML]{FCE4D6}Diffuser & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}52.5$\pm$2.5}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}55.7$\pm$1.3}  & 54.1             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}27.3$\pm$2.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}17.3$\pm$1.9}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2.0$\pm$1.6}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}6.7$\pm$5.7}                          & 13.3                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}123}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}121.5}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}113.9}     & \cellcolor[HTML]{BDD7EE}119.5            \\ \cline{2-14} 
\cellcolor[HTML]{FCE4D6}                                                                                & \cellcolor[HTML]{FCE4D6}AdpDfsr  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}51.8$\pm$0.8}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}55.5$\pm$0.4}  & 53.7             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}8.7$\pm$2.5}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}5.3$\pm$3.4}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}6.0$\pm$3.3}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}12.0$\pm$7.5}                         & 8.0                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}167.9$\pm$5.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}129.9$\pm$4.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}135.1$\pm$5.8} & \cellcolor[HTML]{BDD7EE}144.3            \\ \cline{2-14} 
\cellcolor[HTML]{FCE4D6}                                                                                & \cellcolor[HTML]{FCE4D6}DD       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}75.0$\pm$0.0}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}56.5$\pm$5.8}  & 65.8             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.0$\pm$0.0}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}0.0$\pm$0.0}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}4.0$\pm$2.8}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}8.0$\pm$4.3}                          & 3.0                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}--}        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}--}        & \cellcolor[HTML]{BDD7EE}                 \\ \cline{2-14} 
\cellcolor[HTML]{FCE4D6}                                                                                & \cellcolor[HTML]{FCE4D6}HD       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}71.7 $\pm$2.7} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}73.3$\pm$1.4}  & 72.5             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 83.6$\pm$5.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}--}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{A6A6A6} 88.7$\pm$8.1}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}--}                               & --                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}128.4$\pm$3.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}135.6$\pm$3.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}155.8$\pm$2.5} & \cellcolor[HTML]{BDD7EE}139.9            \\ \cline{2-14} 
\multirow{-5}{*}{\cellcolor[HTML]{FCE4D6}\begin{tabular}[c]{@{}c@{}}Diffusion\\  Planners\end{tabular}} & \cellcolor[HTML]{FCE4D6}DV       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}73.6$\pm$0.1}  & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}94.0$\pm$0.3}  & \textbf{83.8}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}80.0$\pm$1.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}76.4$\pm$2.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}87.4$\pm$1.6}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}89.0$\pm$1.6}                         & \textbf{83.2}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}203.6$\pm$1.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}150.7$\pm$1.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}136.6$\pm$1.3} & \cellcolor[HTML]{BDD7EE}\textbf{163.6}   \\ \hline
\end{tabular}
}
\caption{\textbf{Normalized performance of various offline-RL methods.} DQL* and IQL* are replicated results. Note that the latest version of Antmaze is v2, the previous results on AntMaze-v0 are denoted by gray fonts to differentiate. For our results, data are averaged over 500 episode seeds. We omit the standard errors for simplicity, which however, can be find in the detailed tables in Appendix~\ref{appendix:extensive_results}. The best average performance on each task set are marked in bold fonts. BC: vanilla imitation learning, BCQ: \cite{fujimoto2019off}, CQL: \cite{kumar2020conservative}, IQL: \cite{kostrikov2021offline}, SfBC: \cite{chen2023offline}, DQL: \cite{wang2023diffusion}, IDQL: \cite{hansen2023idql}, DQL* and IDQL*: replicated by \cite{dong2024cleandiffuser}, CEP: \cite{lu2023contrastive}, Diffuser: \cite{janner2022planning}, AdptDfsr: \cite{liang2023adaptdiffuser}, DD: \cite{ajay2022conditional}, HD: \cite{chen2024simple}.}
\label{table:score}
\end{table}

